A Beginner's Guide to Power and Energy Measurement and Estimation for Computing and Machine Learning

Concerns about the environmental footprint of machine learning are increasing. While studies of energy use and emissions of ML models are a growing subfield, most ML researchers and developers still do not incorporate energy measurement as part of their work practices. While measuring energy is a crucial step towards reducing carbon footprint, it is also not straightforward. This paper introduces the main considerations necessary for making sound use of energy measurement tools and interpreting energy estimates, including the use of at-the-wall versus on-device measurements, sampling strategies and best practices, common sources of error, and proxy measures. It also contains practical tips and real-world scenarios that illustrate how these considerations come into play. It concludes with a call to action for improving the state of the art of measurement methods and standards for facilitating robust comparisons between diverse hardware and software environments.

==> inputs/measurement.tex <==
\section{Conducting the Measurement}
\label{sec:measurement}

Once a set of measurements is chosen (some examples are given in Section \ref{sec:system}), the subsequent considerations should focus on refining the measurement process to ensure the highest possible utility of the data while minimizing potential biases or errors introduced by the chosen techniques.

%Here we outline a selection of common pitfalls and trade-offs.

\subsection{Units and Power/Energy Conversion}

When measuring power, it is crucial to understand and manage conversion factors between units, such as Watts (W) to milliwatts (mW) or microJoules ($\mu$J) to Joules (J). For example, tools like pyRAPL report energy in $\mu$J, and your choice of units may depend on your specific use case. You might need to measure CPU energy usage (J), system power draw (W), or battery life (hours), ensuring consistency and compatibility across systems.

Precision is key: use microunits for high precision (e.g., $\mu$J or mW) if required. Additionally, note that some tools provide only power measurements rather than energy.


==> inputs/system.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{pictures/sankey_diagram.svg}
    \caption{This Sankey diagram depicts the power consumption of various system components, with electricity input measured at the wall (left side). The input power supports several components, including the flagship NREL HPC cluster, Eagle. Eagle's power usage is further divided into raw power and the power allocated to an online uninterruptible power supply (UPS), which can be disaggregated by individual nodes (not shown). Note that the proportions of energy distribution are for illustrative purposes only. The online UPS continuously charges and, once fully charged, directs power to the overall system.}
    \label{fig:sankey}
\end{figure}
%DN Says: the below para is super awesome and clear. Thank you to whoever did it.
While the energy consumed by components (or nodes) and background processes should \textit{theoretically} sum to the energy use measured at the wall (Figure \ref{fig:sankey}), many factors that can complicate this relationship including measurement variability, transmission and conversion power losses, interference of the measurement itself, and interference from non-quantified processes.

\subsection{Tradeoffs in Where to Measure}
\label{ssec:where_to_measure}


\begin{figure}
    \centering
    \includegraphics[width=0.55\linewidth]{pictures/diagram.png}
    % \todo{Update figure}
    \caption{ An illustration of scope, control, and accuracy. At the system level, we can measure energy accurately, but lack fine-grained control over how energy was used. At the code level we have detailed high-resolution control over the scope, but have difficulty measuring the impacts of these changes on the wider system.}
    \label{fig:specificity_impact_tradeoff}
\end{figure}



%However, beware that increased power for a shorter duration (e.g. heavily parallelized code) may use less total energy and time since we must move from power estimations to energy estimations. %, in part because of the role of idle power. 
% \todo{the 'however' part doesn't seem to follow on from the absolute vs marginal idea. Maybe it does and i'm not getting it, but if I don't get it someone else might not either-DN.}\todo{Does cooling get measured here? if so lets detail and if not lets add a similar paragraph}



%This method requires detailed instrumentation and can be more complex to implement, but it provides valuable data that can help in optimizing both hardware and software for energy efficiency.

%allows for a more granular analysis of energy consumption and will allow the user to have greater control of estimating the marginal power contribution of their software to a system that is already consuming power natively. This approach 
%By doing so, researchers can gain insights into the energy efficiency of specific hardware and the impact of software optimizations on energy consumption. 


% This decision will depend on the overall goal of your analysis. %\todo{cite the examples we give}.  %Nicole added text to cite examples...
% In the scenario where we are measuring the whole system, the answer is clear, all devices will be included. In fact it may not even be necessary to break down power measurements to different components. \todo[inline]{I think there is some value of talking about on and off device measurments here (mentioned in 2.2.2) as well -NB} 
%\todo[inline]{suggested text to deal with PUE comment below -NB: Even in this situation, there are still additional decisions that can be made. As mentioned above, there is a lot of additional incurred power costs beyond the power consumption of the system. This is often captured by  PUE, or Power Usage Effectiveness. PUE is  the ratio of total amount of energy consumed by the data center and the amount of energy consumed by compute and allows system level measurements to be scaled up for total power estimates.}
%However, in the other scenarios the problem statement defines the specific devices that must be considered. For example, if one is interested in measuring the power or efficiency of fine-tuning vs pre-training it might be useful to track power consumption of both the CPU and GPU while neglecting the contributions of networking between the two. When measuring a particular aspect of the code, measuring the CPU when the code is running on the GPU will simply introduce noise and variability that results in both analysis and conclusions that are needlessly complex. While the decision of what specific devices should be included in the measurement may seem simple, our experience has led us to believe otherwise. 

%\todo[inline]{suggested text on measurement vs estimate is commented here -NB:
%Another important note is that there is a difference between measurement and estimate. Measurements are more accurate than estimates but require access to measurement tools. For example, to measure ''at the wall'' requires access to the data coming from a power meter. However, this power meter measurement is only accurate if the whole system is devoted to running that particular application/job. Otherwise, estimation is needed to isolate the power consumed for a particular workload. In the case of component measurements, many of the tools that exist are estimates or approximations of the power consumed by that component. While there are outliers to this situation where researchers specifically install measurement devices for component level analysis, in most cases component level power measurements are estimates. AJ please add references if text is accepted. here where they actually do install new hardware measurement devices and/or examples of components that have power measurement tools as part of them.}


%The rest of this section will go into details of how the decision of which specific devices will be measured can impact our understanding of the power consumed at the hardware and software level. \todo{maybe we want to foreshadow the rest of the section here -NB}



%However, data centers today use energy to cool, and additional energy to keep the energy stable as it comes off the grid. 

%Grid stability may have large amounts of variability due to fluctuating energy resources and end user demands. %If the computing resource is in a larger facility, like an office or university campus, there are many other users of energy as it comes off of the grid.
%While measuring the utilization of the whole system at the point of power consumption (''at the wall'') is straightforward in its correlation to actual power utilized, it also becomes more difficult to disambiguate any particular contribution of hardware or software configuration. Further, in large scale data centers, the power consumption ''at the wall'' may not be accessible by the user. \todo{Hillary to add some discussion of this here? not sure it is the right place -NB}

%\todo{is this correct? -JG}
%Measuring at the component level, however, allows for a more granular analysis of energy consumption and will allow the user to have greater control of estimating the marginal power contribution of their software to a system that is already consuming power natively. \todo{is this correct? trying to get at the idea of marginal vs absolute which i think is a useful thing to mention. -NB} This approach involves monitoring the power usage of individual components, such as CPUs, GPUs, memory, and storage devices. By doing so, researchers can gain insights into the energy efficiency of specific hardware and the impact of software optimizations on energy consumption. This method requires detailed instrumentation and can be more complex to implement, but it provides valuable data that can help in optimizing both hardware and software for energy efficiency.

%In this context, it is important to consider the following
%\begin{enumerate}
%    \item \textbf{Instrumentation and Tools}: The selection of appropriate tools and instrumentation for measuring energy consumption at the component level is crucial. These tools should be able to accurately capture the power usage of individual components without introducing significant overhead.
%    \item  \textbf{Calibration and Validation}: Ensuring that the measurement tools are properly calibrated and validated is essential for obtaining reliable data. This may involve comparing the measured data with known benchmarks or conducting controlled experiments
%    \todo[inline]{OPEN: I suggest adding another item here around making sure adding the numbers up makes sense and referencing the sampling rate section and the error and variation section. Suggested text commented out -NB\\
%    \textbf{Measurement Compatibility/Scope}: If multiple measurements are being made (usually through measurement of multiple components or multiple full systems) ensure that these numbers can be combined in a way that supports the conclusion. For example, if you are individually measuring CPU and GPU power, adding them together may miss networking costs or may double-count things like data transfers. This might not be an issue if you are interested in comparing two different measurements to each other but may be an issue if you are using the sum of CPU and GPU power to estimate total power consumption.}
%    \item \textbf{Data Analysis}: Analyzing the collected data to identify patterns and insights requires robust data processing techniques. This may include statistical analysis, machine learning algorithms, and visualization tools to interpret the results effectively.
%\end{enumerate}

%On the other hand, measuring power consumption at the wall offers insights into the combined impact of hardware configurations, software workloads, and system settings on energy usage. This information is valuable for identifying opportunities to reduce power consumption, improve performance-per-watt metrics, optimize resource allocation, or create a comprehensive view of energy usage of a system. Measuring power consumption at the wall accounts for inefficiencies in power conversion, distribution losses, and environmental factors (e.g., temperature, humidity) that can affect overall energy consumption. This holistic approach ensures that energy efficiency assessments consider all factors influencing power usage, providing a more accurate representation of the system's environmental footprint. 
%\todo{Somewhere in here we should mention PUE and allude to section 3. } 

\subsection{Component considerations}

\subsubsection{Component measurement granularity}

Within the same device, there may be multiple locations where power measurements can be taken. For example, CPU measurements can be made at the node, socket, core, or even thread level. 
Assuming all threads are equally utilized (which is rarely the case), one should be able to estimate the total amount of CPU node processing power as the number of sockets multiplied by the number of cores multiplied by the number of threads multiplied by the power consumed by one thread.
Similar to the system to code level of measurement (Figure~\ref{fig:specificity_impact_tradeoff}), the node level measurements provide the most accurate measurements of power and thread level the least. While a solid experimental design and hypothesis can help control for ambiguity and aide in interpretation of, say, thread measurements, we recommend measuring at the highest level of granularity that will support your measurement goals.

\begin{tipbox}
\textbf{Tip!} Measure at the highest level component granularity that will support measurement goals. For example, choose node-level over thread-level, as node-level has a designated register for power, and thread-level measurements could require the use of a proxy.  
\end{tipbox}

\begin{scode}
    \textbf{Real world learning (S3):}
    In our experiments to understand the impact of parallel data loading with specific number of threads, the total energy used was lower than when single thread was being used. This higher energy consumption of the single thread case was due to idle cost. The surprising aspect we found 
    was that multiple threads was not multiplicatively less than a single thread. This shows that thread level analysis can be difficult to understand.
    
    %that overall power consumption when using multiple threads for data was not multiplicatively less than a single thread power consumption. This showed that using multiple threads add to the complex thread switching that adds to the over power consumption. This is true, eventhough all the threads in question are releated to the same experiments. 
    
\end{scode}%, we can develop baseline measurements, have a controlled environment, do statistical analysis to analyze the variability, and adjust sampling frequency based on observed variability. 

%\todo[inline]{Advice on when to pick one vs other? Or at least advice to standardize?}
% \todo[inline]{It might be useful to have a picture here. Latex has link to one I found that we could redraw} %https://www.google.com/url?sa=i&url=https%3A%2F%2Fchunjie-sam-liu.life%2Fen%2Fpost%2F2019-08-15-r-parallel-computation%2F&psig=AOvVaw2qYGc3tYcIs2HTdFIYzMrU&ust=1720125226836000&source=images&cd=vfe&opi=89978449&ved=2ahUKEwj-gpj624uHAxVCPDQIHaPdDewQjRx6BAgAEBU}
%Similar to the system to code level trade-off of figure~\ref{fig:specificity_impact_tradeoff}, as one estimates power consumption of smaller components of an overall chip, the accuracy and reliability of these measurements decrease.

%Generally speaking, node level measurements/estimates approximate the energy consumed by a motherboard, which may contain multiple sockets. The socket measurements/estimates captures all cores of the CPU and all threads running on any of these CPU cores. CPU core measurements/estimates allow one to capture the energy consumption of multiple threads that are potentially doing different amounts of computation and provides a more granular understanding than the socket level. Thread level estimates are the most granular but also the most difficult to estimate and trust. While tools do exist to estimate thread level power consumption\autocite{newsom2016thread}, one must have a strong understanding of the hardware specifications and system configuration and have a meaningful experimental design such that comparisons between situations can be trusted %\todo{This is very vague}. 

%Because of the increasing need for estimation, and the increasing error in these estimations as you move from node, to socket, to core, and finally to thread, we recommend measuring at the highest level of granularity that will support your measurement goals.


% AJ do we have an actual example of where we got caught up in measuring an epoch here? I know we considered all sorts of different measurement level, what did we chose and why?

% SOVAN please add a S3 box here about your Transformer thread comparison experiment, highlighting the challenge of getting a meaningful comparison

% \todo[inline]{Optional add real world S1 story here about how cpu + gpu might not capture all the information but might still be enough}


% \todo[inline]{Optional add real world S1 story here about how cpu + gpu might not capture all the information but might still be enough}


%\subsection{At the wall}



==> inputs/walkthroughs.tex <==

\chapter{Power Estimation Scenario Walkthroughs}
Below, we outline a series of scenarios and walk through the relevant factors to consider, beyond the basic formula outlined above.

\section{Scenario 1: Comparing Software Versions}
\textit{I want to see how one complete piece of software compares to another so I can figure out which is the less consumptive version to put into production.}
\begin{enumerate}
    \item Define the problem:
    \begin{enumerate}
        \item Determine the metrics you’ll use as comparison. If you are measuring power consumption of the CPU making network requests, you may want to define your results as amount of power consumed per n number of requests.
        \item Define the system level you be conducting your measurements. Are you trying to measure the power consumption of your software when it runs on a specific device, or of the entire system as the application runs? In some cases, availability of energy measuring tools might determine the system level you examine.
    \end{enumerate}
    
    \item Particularly relevant tools:
    \begin{enumerate}
        \item Benchmarks or benchmarking tools to measure software performance metrics, like transactions per second watt hour, or inference accuracy, to enable you to put the energy consumption into context of the work the software does.
    \end{enumerate}

    \item Proxy considerations:
    \begin{enumerate}
        \item If access to physical hardware is not possible to get energy measurements, it may be possible to use GPU/CPU utilization as a proxy. But if you are still struggling to isolate per-application use, you may have to redefine the problem. 
        \item It is possible to use \hyperref[memory]{memory usage} as a proxy. 
    \end{enumerate}

    \item Scope of Measurement:
    \begin{enumerate}
        \item System measured is defined as part of the problem definition; ensure the scoping remains consistent across software measured.
    \end{enumerate}

    \item Common mistake areas:
    \begin{enumerate}
        \item Don’t simply measure the power consumption of each application. You more likely want to compare the power consumption with respect to performance. 
    \end{enumerate}

    \item Relevant Sources of \hyperref[error]{Error}:
    \begin{enumerate}
        \item Background processes may affect measurements.
    \end{enumerate}

    \item Comparison Scope:
    \begin{enumerate}
        \item Compare work that was generated using the same methodology on the same hardware system.
        \item Energy consumption comparisons should also take into account performance differences or any changes in software features.
    \end{enumerate}
\end{enumerate}

\section{Scenario 2: Identifying Inefficient Features Code Sections}
\textit{I want to identify a specific branch of my code, function call, or process training, to pinpoint where I can improve efficiencies.}
\begin{enumerate}
    \item Define the metrics:
    \begin{itemize}
        \item Identify what piece of the code you are looking to evaluate and what characteristics of that work are you trying to measure. For example, we could measure the total energy of doing the work, or we could measure relative to performance (i.e. number of requests per second per watt hour)
        \item In cases where direct power measurements are unavailable via meters or software tools, pinpoint the critical hardware components involved in the work and select an appropriate proxy for energy consumption. This could involve identifying components such as the CPU, GPU, or memory, and using metrics like CPU utilization, GPU utilization, or memory bandwidth as proxies for energy consumption.
    \end{itemize}
    
    \item Particularly relevant tools:
    \begin{itemize}
        \item N/A
    \end{itemize}
    
    \item Proxy considerations:
    \begin{itemize}
        \item N/A
    \end{itemize}
    
    \item Scope of measurement:
    \begin{itemize}
        \item Energy consumption during different phases of the workflow (e.g., data processing, computation, I/O operations).
        \item Resource utilization across hardware components (CPU, GPU, memory) during task execution.
        \item Differentiate between system-level power consumption and component-level power consumption.
    \end{itemize}
    
    \item Common mistake areas:
    \begin{itemize}
        \item Avoid measuring very short-duration events (less than approximately 0.1 seconds) as they may introduce inaccuracies due to the power associated with the measurement process itself.
        \item If you are working in a hyperthreading environment, reaching over 100\% utilization is expected behavior because it is possible to double count. Make sure you know how many threads you are using and how they are distributed among the cores. For more information see this \href{faq}{FAQ}.
        \item Evaluate energy efficiency optimizations comprehensively, considering factors beyond simple parameter changes.
        \item Always establish a baseline for comparison when evaluating the impact of optimizations.
    \end{itemize}
    
    \item Relevant Sources of \hyperref[error]{Error}:
    \begin{itemize}
        \item Variability in workload characteristics or data inputs may influence energy consumption and performance metrics.
        \item Hardware variations across different systems or environments can lead to inconsistencies in measurements.
        \item If the piece of code we are trying to measure doesn’t run long enough (in most cases, we would want to measure something that runs longer than 0.1 seconds), power measurement tools might not be capable of measuring accurately for short durations.
    \end{itemize}
    
    \item Comparison Scope
    \begin{itemize}
        \item Always compare back to a baseline measurement.
        \item Only measurements from the same system should be compared when evaluating the efficiency of a specific section of code.
    \end{itemize}
\end{enumerate}

\section{Scenario 3: Tracking Development Process Efficiency}
\textit{I want to track my development processes (building, testing, change management, etc.) so I can see across a long-term workflow if there are more energy-consumptive parts that I can change.}
\begin{enumerate}
    \item Define the metrics:
    \begin{itemize}
        \item Identify the different segments of your development process you would like to profile (i.e. development tools, third-party apps \& service, code execution, Continuous Integration/Continuous Development, database infrastructure, etc.)
    \end{itemize}
    
    \item Particularly relevant tools:
    \begin{itemize}
        \item Your current infrastructure might already have an energy profiling mechanism. Tools such as Dynatrace and Grafana may already provide the ability to measure energy consumption of your development process. Sometimes these values are not as granular as we would like (perhaps they report for the entire system rather than your one application) but check to see if these might meet your requirements.
    \end{itemize}
    
    \item Proxy considerations:
    \begin{itemize}
        \item In some cases, you might want to track energy consumption on infrastructure that you might not have direct access to. For example, if employing GitHub actions as part of your CICD flow, your code might be running on containers on an external platform. In those cases, use CPU utilization or GPU utilization.
    \end{itemize}
    
    \item Scope of measurement:
    \begin{itemize}
        \item Energy consumption during development phases (build, test, deployment).
    \end{itemize}
    
    \item Common mistake areas:
    \begin{itemize}
        \item Ignoring the impact of external factors (e.g., system updates, changes in third-party dependencies) on energy consumption over time.
        \item Looking too closely at raw numbers will introduce a lot of noise. There can be a lot of changes and fluctuations happening in background processes that you may not be aware of that will affect energy consumption. Look for general trends in the data rather than a hard increase or decrease.  
        \item Don’t attempt to compare different stages of the development process with each other or with an apparently similar workflow without fully considering whether the process in question has higher or lower energy requirements. 
    \end{itemize}
    
    \item Relevant Sources of \hyperref[error]{Error}:
    \begin{itemize}
        \item Incomplete data due to incomplete integration with development tools.
        \item Variability in development environments.
    \end{itemize}
    
    \item Comparison Scope
    \begin{itemize}
        \item Energy consumption trends over time.
        \item Impact of code changes on energy.
    \end{itemize}
\end{enumerate}

\section{Scenario 4: Comparing Software Energy Consumption while Using Unknown Hardware}
\textit{I am running my software in a serverless environment (like Google Cloud Platform [GCP]) and want to compare my software with another piece of software.}
\begin{enumerate}
    \item Define the metrics:
    \begin{itemize}
        \item Clearly define the specific aspects of energy consumption you want to compare, such as CPU usage, memory usage, disk I/O, and network activity. Determine whether you're interested in overall energy consumption or specific components contributing to it.
    \end{itemize}
    
    \item Particularly relevant tools:
    \begin{itemize}
        \item Profiling tools for software performance, to facilitate comparability between the two pieces of software.
    \end{itemize}
    
    \item Proxy considerations:
    \begin{itemize}
        \item Depending on what you are trying to measure, you could employ energy profiling tools to measure the energy consumption to get an overview of the entire system.
        \item It may be possible to use GPU/CPU utilization as a proxy if there is no way to directly access the hardware.
    \end{itemize}
    
    \item Scope of measurement:
    \begin{itemize}
        \item If possible, try profiling the software performance across multiple hardware configurations. This will give a more holistic understanding of how the software performs in various environments.
    \end{itemize}
    
    \item Common mistake areas:
    \begin{itemize}
        \item Avoid estimating or assuming hardware characteristics based solely on software performance metrics. Consider external factors that may influence energy consumption, such as background processes, system configuration, and workload characteristics. Try to isolate the impact of these factors to ensure a fair comparison.
    \end{itemize}
    
    \item Relevant Sources of \hyperref[error]{Error}:
    \begin{itemize}
        \item Inaccurate hardware simulation models.
        \item Variability in software execution environments.
    \end{itemize}
    
    \item Comparison Scope
    \begin{itemize}
        \item As much as possible create a standardized testing environment to ensure fair comparison. This environment should include the same operating system and workload conditions for both software systems. If you can't replicate the exact hardware configuration, try to match it as closely as possible in terms of performance characteristics.
        \item Energy consumption trends on different hardware configurations.
        \item Relative performance on known hardware.
    \end{itemize}
\end{enumerate}

\section{Scenario 5: Testing Software Energy Consumption on Different Hardware}
\textit{I want to test if my software consumes more energy on one type of hardware versus another.}
\begin{enumerate}
    \item Define the metrics:
    \begin{itemize}
        \item Choose appropriate metrics for measuring energy consumption. These metrics could include total energy consumption (measured in Joules), average power usage (measured in Watts), or energy efficiency metrics like performance per watt. Ensure these metrics are consistent and comparable across different hardware configurations. 
        \item Break down the unit of work to test, eg. energy consumption per inference, per training epoch, etc.
    \end{itemize}
    
    \item Particularly relevant tools:
    \begin{itemize}
        \item No particular tool stands out in this scenario but ensure the tools you use work across the different hardware being tested.
    \end{itemize}
    
    \item Proxy considerations:
    \begin{itemize}
        \item N/A
    \end{itemize}
    
    \item Scope of measurement:
    \begin{itemize}
        \item Energy consumption on hardware configurations being tested.
        \item Software performance metrics on each hardware setup.
    \end{itemize}
    
    \item Common mistake areas:
    \begin{itemize}
        \item Neglecting to account for differences in workload distribution across hardware configurations.
        \item Take into account external factors that may influence energy consumption, such as hardware utilization, workload distribution, and power management settings. Normalize energy consumption data to account for these factors and ensure fair comparisons.
        \item Be careful about comparing raw numbers. Draw conclusions about the impact of different hardware configurations on software energy consumption based on the full analysis of energy consumption data. Identify hardware types that exhibit higher or lower energy efficiency and provide recommendations for optimization or hardware selection based on the findings.
    \end{itemize}
    
    \item Relevant Sources of \hyperref[error]{Error}:
    \begin{itemize}
        \item Variability in hardware performance across time due to hardware degradation.
        \item Inconsistencies in workload distribution.
    \end{itemize}
    
    \item Comparison Scope
    \begin{itemize}
        \item Energy consumption per unit of work on different hardware.
        \item Relative performance across hardware configurations.
    \end{itemize}
\end{enumerate}


==> inputs/walkthroughs_ak.tex <==

\section{Power Estimation Situations Walkthroughs}
Below, we outline a series of situations and walk through the relevant factors to consider.

\subsection{Situation 1: Comparing Software Versions}
\textit{I want to see how one complete piece of software compares to another so I can figure out which is the less consumptive version to put into production.}
\begin{enumerate}
    \item Define the metrics: Identify the comparison metrics (e.g., power per number of requests) and specify the system level for measurement (e.g., specific device or entire system). In some cases, the availability of energy measuring tools might determine the system level you examine.
    
    \item Tool requirements: Look for benchmarking tools that measure performance metrics like transactions per watt hour.

    \item Interpretation: Consider analyzing the idle vs active trade-offs. One configuration may have a higher standby power but lower per-request energy than another. Which one is less consumptive will depend on the frequency (and perhaps distribution) of the requests.

    % \item Proxy considerations: Component level resource utilization is acceptable as a proxy. 

    \item Challenges/Common Mistakes: Avoid comparing power consumption without considering performance. Additionally, be mindful of double-counting aspects of a job across different system configurations. Consider the standby or idle power consumption and the additional marginal energy cost per action such as requests serviced or epochs trained.

\end{enumerate}

% \textbf{Real-World Example:} While comparing transformer and LSTM architectures, we estimated CPU and GPU power through independent functions with the same sampling rate. Even though power estimations were sometimes slightly out of sync, the analysis showed transformers took less time than LSTMs in pre-processing batches, indicating potential efficiency improvements for LSTMs.

\subsection{Situation 2: Identifying Inefficient Features Code Sections}
\textit{I want to identify a specific branch of my code, function call, or process training, to pinpoint where I can improve efficiencies.}
\begin{enumerate}
    \item Define the metrics: Identify which parts of the software are under evaluation. This could include algorithms, data structures, or overall software architecture.

    \item Tool requirements: Look for tools that can do energy profiling of isolated code sections or from specific software/hardware components.
    
    \item Interpretation: Compare energy usage across different architectures or design patterns. Consider factors like algorithm efficiency, data access patterns, and system interactions.

    \item Challenges/Common Mistakes: Not accounting for the energy consumption of other parts of the workload can introduce high, confounding noise into your measurements. For example, a part of the workload not under study may have a variable impact on the measurements you are using (i.e. CPU/GPU resource utilization) which can skew your comparisons.

\end{enumerate}

\subsection{Situation 3: Tracking Development Process Efficiency}
\textit{I want to track my development processes (building, testing, change management, etc.) so I can see across a long-term workflow if there are more energy-consumptive parts that I can change.}
\begin{enumerate}
    \item Define the metrics: Determine the stages of the development process to be measured, such as code compilation, testing, or continuous integration pipelines.
    
    \item Tool requirements: Several tools may be needed to cover the different aspects of the development process. Look for tools built into your existing infrastructure that can measure energy consumption.

    \item Interpretation: Analyze the energy consumption data to identify stages or tasks that are energy-intensive. Look for trends over time rather than focusing on single measurements.
    
    \item Challenges/Common Mistakes: Consider the impact of external factors (e.g., system updates, changes in third-party dependencies) and hardware. 
\end{enumerate}

\subsection{Situation 4: Comparing Software Energy Consumption while Using Unknown Hardware}
\textit{I am running my software in a serverless environment (like Google Cloud Platform [GCP]) and want to compare my software with another piece of software.}

\begin{enumerate}
    \item Define the metrics: Identify which hardware components are being compared, such as different CPUs, GPUs, or entire server configurations.
    
    \item Methodology/Tool requirements: Define a standardized methodology to measure power consumption regardless of different underlying hardware configurations. For example, if hardware changes between measurements, try to map a common configuration. Standardize the CPU utilization and runtime numbers based on the number of cores and clock speed.
    
    \item Interpretation: Compare energy consumption, performance per watt, and other relevant metrics. Consider factors like hardware utilization, thermal characteristics, and system interactions.
    
    \item Challenges/Common Mistakes: Avoid estimating or assuming hardware characteristics based solely on software performance metrics. Consider external factors that may influence energy consumption, such as background processes, system configuration, and workload characteristics. Try to isolate the impact of these factors to ensure a fair comparison.
\end{enumerate}

% \textbf{Real-world Example:} Researchers compare the energy efficiency of a high-performance CPU against a low-power CPU for a specific workload. They analyzed how different hardware configurations impact overall energy consumption and performance.

\subsection{Situation 5: Testing Software Energy Consumption on Different Hardware}
\textit{I want to test if my software consumes more energy on one type of hardware versus another.}
\begin{enumerate}
    \item Define the metrics: Determine which applications or application components are being evaluated. This could include web services, desktop applications, or mobile apps.
    
    \item Tool requirements: When possible, use tools that can work across different software/hardware to ensure some level of consistency in the measurement.

    \item Interpretation: Draw conclusions about the impact of different hardware configurations on software energy consumption based on the full analysis of energy consumption data. Identify hardware types that exhibit higher or lower energy efficiency and provide recommendations for optimization or hardware selection based on the findings.

    \item Challenges/Common Mistakes: Account for varying standby power consumption. Some components may have higher peak throughput but also higher standby power usage. For certain workloads, these systems are more efficient because they complete tasks quickly despite higher power draw. However, workloads that do not fully utilize these systems (e.g., single-threaded tasks on a single-core CPU vs. a multi-core CPU) will be less efficient, as they will run for a similar duration but consume more baseline power.

\end{enumerate}

